A3D: Does Diffusion Dream about 3D Alignment?

We tackle the problem of text-driven 3D generation from a geometry alignment perspective. Given a set of text prompts, we aim to generate a collection of objects with semantically corresponding parts aligned across them. Recent methods based on Score Distillation have succeeded in distilling the knowledge from 2D diffusion models to high-quality representations of the 3D objects. These methods handle multiple text queries separately, and therefore the resulting objects have a high variability in object pose and structure. However, in some applications, such as 3D asset design, it may be desirable to obtain a set of objects aligned with each other. In order to achieve the alignment of the corresponding parts of the generated objects, we propose to embed these objects into a common latent space and optimize the continuous transitions between these objects. We enforce two kinds of properties of these transitions: smoothness of the transition and plausibility of the intermediate objects along the transition. We demonstrate that both of these properties are essential for good alignment. We provide several practical scenarios that benefit from alignment between the objects, including 3D editing and object hybridization, and experimentally demonstrate the effectiveness of our method. https://voyleg.github.io/a3d/

==> Makefile <==
export TEXINPUTS = ./src/aux:
export BSTINPUTS = ./src/aux:
export TEXMFOUTPUT = ./build:
SOURCES = $(shell find . -name '*.tex' -type f) $(shell find src/img -type f)
$(info $$SOURCES is [${SOURCES}])

.PHONY: all, clean

all: build/main.pdf

clean:
	rm -rf build

build/main.pdf : build/%.pdf: $(SOURCES)
	mkdir -p build
	pdflatex --shell-escape -output-directory=build $*.tex
	bibtex build/$*
	pdflatex --shell-escape -output-directory=build $*.tex
	[ -e ./build/$*.bbl ] && pdflatex --shell-escape -output-directory=build $*.tex

build/main_opt.pdf : build/%_opt.pdf : build/%.pdf
	ghostscript -dNOPAUSE -dQUIET -dBATCH -sDEVICE=pdfwrite \
	-dPDFSETTINGS=/prepress \
	-dPrinted=false \
	-dPassThroughJPEGImages=false \
	-dColorImageResolution=300 \
	-dGrayImageResolution=300 \
	-sOutputFile=$@ $<


==> src/main/plan.tex <==
1. Problem statement: Joint Generation of the Aligned 3D models [set of textual prompts -> set of 3d models]
2. Application: Creation of the collection of the aligned 3D models, for further use in the computer graphics pipeline. Side applications: Hybridisation (object composition), 3D editing.

- Declare and explain "structural alignment"

3. Motivation (Related work). Three threads of work can be adapted for aligned generation.
    1. Text-to-3D generation
        - Produces 3D models separately from each other and due to the properties of the diffusion models the results are ill aligned in the terms of the corresponding structural parts
        - We support this with our motivation figure 2 and the results of ablation study.
    2. Large 3D generative models
        -  Plethora of work trains a feedforward network with SDS to produce 3D model given a textual prompt. Due to the mode seeking behavior of SDS there is no guarantee for geometric alignment and often these methods produce misaligned objects.
    3. 3D editing
        - Produces the 3D objects sequentially, but has the drawback, since it operates with the given asset and lacks the flexibility of the joint optimization, which leads to a low quality of the generated results.
        - We support this with our comparison with the respective methods.
        - Maybe, we can add a row to the motivation figure 2 with 5 objects sequentially generated with MVEdit.

4. Related work (b). Research on generative models (GAN's and autoedcoders) shows that alignment between the generated objects can be improved with regularization of the linear transitions between the latent codes, which leads to better FID, disentanglement.
1) StyleGAN directly regularize the perceptual length of the trajectory in the images space. Unlike this we implicitly regularize the smoothness of the intermediate objects.
2) (Goodfellow et al) adversarial optimizes the plausibility of the samples from the interpolated latent codes. Unlike this we use SDS as a critic. 
Unlike these models our latent space consists of the set of the discrete objects and transitions between them.

5. a) Our method embeds the set of the 3D objects in the joint latent space on par with the transitions between the pairs of this objects. We jointly optimize both the boundary points and the transitions from two perspectives
    - The intermediate points in the transitions should look plausible. For this, we employ the SDS as a critic.
        - To show that this is important, we do an ablation study where we train a single network but w/o optimization of the trajectory.
          Such intermediate version of the method produces results that are aligned worse qualitatively, maybe also quantitatively.
    - The transitions should be smooth. For this we [implicitly] regularize the smoothness of the intermediate objects by using a network with a low capacity.
        - To show that this is important, we do two ablation experiments.
            - We increase the number of layers in our network, which relaxes the regularization on the smoothness.
              (We expect that) This version of the network produces results with worse alignment.
            - We vary the smoothness penalty.

6. b) As a side application our method allows to seamlessly sew up two produced models through the bilinear interpolation of the latent codes between the keypoints. The second application is 3D editing which is achieved by fixing one point on the trajectory with the photometric anchor loss. 

7. We demonstrate the capabilities of our method in three tasks.
   In aligned generation and editing we evaluate our method quantitatively and compare with competitors.
   For hybridization we just show our results.
   We implement our method based on MVDream backbone, it uses NeRF as 3D representation. In supllementary we show some results of our method implemented on RichDreamer backbone, which uses DMTet. Add "teaser" of the new results in the main

8. We quantify three kinds of properties:
    - Alignment of corresponding structural parts of generated objects - DIFT score.
    - Text-3D alignment - GPTEval (Text-Asset Alignment, Text-Geometry Alignment), CLIP.
    - Asset Quality - GPTEval (3D Plausibility, Texture Details, Geometry Details, Overall).

9. Results of Aligned generation.
    1. We make a collection of the prompt pairs which describe objects which are similar morphologically, but differs geometrically.
    2. Since there are no methods for generation of collections of objects with publicly available implementation, we compare with set of state-of-art 3D editing methods in the following setup - we generate the initial object from the first prompt and then edit it with the second prompt. Then we repeat the process in the inverse direction. We consider both versions of results.
    3. Our results:
        - Our method shows good structural alignment (on par with MVEdit), as confirmed with DIFT-alignment,
        - while at the same time outperforming the competitors in the terms of alignment with the prompt,
        - and the overall asset quality
        - due to the ability to optimize not only the result but also the "source" object.
        - We show RGB and grayscale renders, for competing methods show only one-way pair of the results (the rest --- in supplementary).
          Initially, show the same four pairs of objects as in NeurIPS version, later Savva maybe picks different objects.
        - Compared with MVEdit our method produces more detailed geometry, and compared with LucidDreamer our geometry is less noisy.
        - MVEdit, using just one text prompt for the generation of the initial model, often produces the model that is hard to transform to be consistent with the second prompt. We emphasize that this is a usual behaviour for MVEdit, see the results in supplementary.


10. Results of Pose-preserving transformation.
    1. We collect a set of the 3D models from the internet open sources including both the textured and textureless meshes for the better test of the real-life applications. For each mesh we produce a prompt describing which object we want to obtain.
    2. We generate results both for our method and for the competitors, evaluating on the same set of metrics.
    3. Our results:
        - Generally we produce results on par with the state-of-art editing methods
        - Compared with MVEdit our method
            - produces more detailed results, (confirmed by GPTEval)
            - adds details to the object based on the prompt, e.g "dwarf with an axe", "jedi with lightsaber", "princess on a throne", (confirmed by GPTEval Text-X Alignment)
            - this leads to a slightly worse DIFT-alignment metric
        - While LucidDreamer produces more detailed results then our method, their results are rarely aligned with the source mesh, have inconsistent structure, and suffer from "Janus face" problem (see supplementary videos)
        - We don't compare with LucidDreamer quantitatively since it diverges for a half of the scenes (maybe in supplementary show the DIFT-alignment per scene, w/o any comments).
        - We show RGB and grayscale renders. Initially, show the same four pairs of objects as in NeurIPS version, later Savva maybe picks different objects.


11. Hybridisation.
    - We demonstrate the ability of our method to seamlessly sew up the parts of the generated objects in the Frankenstein style, through the smooth interpolations of the latent codes.
    - Remarkably, our approach allows us to easily transition between the objects in places with different geometries, \eg, the necks of the gopher and kangaroo, which have different diameters, or waists of the seahorse and mermaid, which have different other parts of the object nearby. This is in contrast to methods like MVEdit that produce triangular meshes, which have to be locally aligned first to be stitched together.


-----> PROCEED HERE when we have the results of ablation study

12. Ablation 1. We generate the objects separately from each other.
    - 


ii) We generate the objects jointly but without optimizing trajectory. iii) We learn the trajectory with the empty prompt. iiii) We increase the capacity of the model. iiiii) We vary the smoothness penalty.



-------------
Supplementary
-------------
1. Aligned generation with RichDreamer
    - Similar structure to Aligned generation in the main text
    - Show quantitative and qualitative results and say that with this backbone we also obtain good results but a different trade-off between the alignment and the quality of the generated objects.
2. We do not show anything else for RichDreamer and if the reviewers ask for the results in different tasks, Savva expects to be able to get them during the rebuttal period.
